Evaluating COVID-19 Surveillance Testing Strategies at Colorado School of Mines: A Stochastic Modeling Approach

This study introduces a stochastic model of COVID-19 transmission tailored to the Colorado School of Mines campus and evaluates surveillance testing strategies within a university context. Enhancing the conventional SEIR framework with stochastic transitions, our model accounts for the unique characteristics of disease spread in a residential college, including specific states for testing, quarantine, and isolation. Employing an approximate Bayesian computation (ABC) method for parameter estimation, we navigate the complexities inherent in stochastic models, enabling an accurate fit of the model with the campus case data. We then studied our model under the estimated parameters to evaluate the efficacy of different testing policies that could be implemented on a university campus. This framework not only advances understanding of COVID-19 dynamics on the Mines campus but serves as a blueprint for comparable settings, providing insights for informed strategies against infectious diseases.

==> outline.tex <==

\section{Introduction}
 \begin{itemize}
        \item Background of COVID-19, what is it, when did it start
        \item Covid on college campus response, campuses shut down and were remote
        \item Purpose of the study.. Explanation of the need for a stochastic compartmental model of COVID-19 on a college campus
        \item Discussion of the potential benefits of such a model, such as its ability to predict the spread of COVID-19 under different scenarios and the potential for identifying effective testing strategies
        \item Our goal is to create a stochastic model of the spread of COVID-19 on the Colorado School of Mines campus using an approximate method to fit the model to campus case data. Then, we use this model to simulate different testing strategies to test the effectiveness of different policy decisions on the spread of the disease on campus.
        \item Previous studies on COVID-19 modeling on college campuses
        \item Description of SEIR models and their applications in infectious disease modeling
        \item ODE models with pros and cons
        \item Discrete stochastic model advantages
        \item $R_0, \beta$ disucssion.. what are these metrics and what do they mean for disease spread
        \item models with testing strategy and quarantine
        \item Introduction to the ABC method and its use in fitting models to data
        \item how are mathematical/stats models being used by policy makers 
        \item Discussion of the potential benefits of such a model, such as its ability to predict the spread of COVID-19 under different scenarios and the potential for identifying effective testing strategies


\end{itemize}


\section{Methods}
\subsection{Study area}
- Background on Mines, location in Golden, CO. Size of population, breakdown of on-campus/off-campus, graduate population

- Fall 2020 classes 70\% in person


Colorado School of Mines partnered with COVIDCheck Colorado (CCC), a social benefit enterprise of the Gary Community Investment Company, to implement a COVID-19 surveillance testing program on the Mines campus \cite{ccc}. Results were guaranteed to be returned within 48-72 hours.  All students living on campus, athletes, and some face-to-face faculty were included in the surveillance testing pool and being tested every two weeks.  Any student exhibiting symptoms could be tested either through CCC or though the Student Health Center. 

\subsection{Data}
- Data on student body distribution

- Class schedule data for connection

- Case data by student type

%- Vaccination data?

- \textbf{Figure of cases time series, discuss why the data is difficult, multiple peaks, etc}

\subsection{Model}



%The number of individuals that transition


\subsection{Parameters and Transition Probabilities}





\subsection{Equations}


\subsection{Next Generation Matrix}



\subsection{Parameter Estimation via Approximate Bayesian Computation}


\subsection{Testing Strategy Simulation}



\subsection{Policies to test/compare}

- change testing frequency

- change number of people tested

- change quarantine # and quarantine duration

\section{Results}

- Simulation study results/sensitivity?

- Model output vs data

- Heatmap of ABC metrics fitting

- results of simulating different policy decisions


\section{Discussion}

- How our results are useful for policy makers

- Discuss how diff param values/policy decisions change things

- Challenges/limitations of our study

- how could this framework be used to study other diseases?



* Note: Look back at Response to a COVID-19 outbreak on a college campus figure 2 for potential testing with cases plot, bar colors by type of student 


